How well can machine-generated texts be identified and can language models be trained to avoid identification?

With the rise of generative pre-trained transformer models such as GPT-3, GPT-NeoX, or OPT, distinguishing human-generated texts from machine-generated ones has become important. We refined five separate language models to generate synthetic tweets, uncovering that shallow learning classification algorithms, like Naive Bayes, achieve detection accuracy between 0.6 and 0.8. Shallow learning classifiers differ from human-based detection, especially when using higher temperature values during text generation, resulting in a lower detection rate. Humans prioritize linguistic acceptability, which tends to be higher at lower temperature values. In contrast, transformer-based classifiers have an accuracy of 0.9 and above. We found that using a reinforcement learning approach to refine our generative models can successfully evade BERT-based classifiers with a detection accuracy of 0.15 or less.

==> 2-related_work_old.tex <==
\section{Related Work}

% Literature overview of detection models
To detect synthetically generated text, we first use simple state-of-the-art models such as naive Bayes classifiers or support vector machines to represent the Bag-of-Words classification approach. We then proceed with BERT \parencite{DBLP:conf/naacl/DevlinCLT19} models that have undergone a transfer learning process to become a classifier for machine-generated texts. Other transformer models, such as the RoBERTa Base OpenAI Detector, have successfully been used to detect GPT-2 generated content \parencite{solaiman2019release}.

Classifiers like RoBERTa or BERT-based ones have certain drawbacks, like their tendency to over-fit and the requirement of training a classification model every time a new generator is released. To address this issue, zero-shot classifiers like DetectGPT \parencite{DBLP:journals/corr/abs-2301-11305} have been developed, which only need a copy of the model to be tested and a second language model to introduce random permutations to the test string. As they rely on introducing random permutations to the test string, they cannot function with a short input string.

Due to the novelty of most classification approaches, there are few scientific publications on bypassing them, like the paraphrasing-based one from \textcite{DBLP:journals/corr/abs-2303-13408}. Since we use reinforcement learning to adjust our generative model to bypass the classifier, our approach is based on the paper \enquote{Fine-Tuning Language Models from Human Preferences} by \textcite{DBLP:journals/corr/abs-1909-08593-neu}.

% Generative approaches
As a foundation of the generative part of our experiments, we use the GPT-based models GPT-Neo-125M, GPT-Neo-1.3B, GPT-Neo-2.7B \parencite{gpt-neo}, GPT-J-6B \parencite{gpt-j}, OPT-125M, OPT-350M, OPT-1.3B, OPT-2.7B \parencite{zhang2022opt} and GPT-2 \parencite{radford2019language}.


Transformer reinforcement learning is a versatile approach that can be used with other types of LLM-generated content. Although the linguistic refinement stage is not mandatory due to the comparison with a reference model in transformer reinforcement learning, it can help enhance the generated output. For instance, when generating source code, the refinement stage may check if the code executes without any errors. For the purpose of this paper, we will focus solely on creating fake tweets.

Our study focuses on reinforcement learning, a technique that allows models or agents to learn how to maximize rewards without labeled data. However, training can be challenging due to the unstable characteristic of reinforcement learning in combination with large language models. Our approach addresses these challenges, and the generated output of the fine-tuned model does not require extra steps, like using synonyms to bypass a classifier. This is the main difference from other approaches based on the obfuscation built into the language model after successful reinforcement learning.


==> 3-dataset.tex <==
\section{Data set}
To improve the quality of the language model, filters are recommended to be applied to the raw Twitter data stream before training. This is because Twitter has a lot of spam and advertising content. During the collection of the data set from January to February 2020, spam content was particularly prevalent. However, with fewer people accessing the Twitter API today, it may not be as big of an issue.

% We applied filter policies to improve training data accuracy, but some events had a significant impact due to their volume. See Table \ref{tab:dataset-filter_policies} for policy details.

We applied the following filter policies to improve training data accuracy: \textit{a)} Verified users (i.e., prominent users or institutions), \textit{b)} English Language (for pragmatic evaluation purposes with other state-of-the-art literature), \textit{c)} Non-truncated tweets (since long tweets get truncated if not requested in full length, an undesirable property for training), \textit{d)} Original tweets (omit quotes, replies, or retweets to generate unique texts), \textit{e)} no celebrity accounts (since accounts with $\geq100.000$ followers are often used to promote products and services) and \textit{f)} normal tweet volume to avoid spam content (filter users with at most 20 tweets per day).

Overall, the data set consists of $k = 2.000.000$ tweets from $n = 136.450$ real accounts and is split into two equal parts, one for the transfer learning of the language models and one for testing the classificators. Creation and splits of the data set are illustrated in Figure \ref{fig:flowchart}.


% \begin{table*}[t]
% 	\center
% 	\caption{Filter Policies for Training Data}
% 	\begin{tabular}[t]{l|l}
% 	    \textbf{Policy} & \textbf{Note} \\
%         \hline
%         Verified Users & Restrict on verified, i.e., prominent users or institutions.\\
%         English Language & For pragmatic evaluation purposes with other state-of-the-art literature. \\
%         Non-Truncated Tweets & Long tweets get truncated if not requested in full length, an undesirable property for training. \\
%         Only original Tweets & Omit quotes, replies, or retweets to generate unique texts. \\
%         No Celebrity Accounts & Prominent accounts ($\geq$ 100.000 followers) are often used to promote products and services. \\
%         Normal Tweet Volume & To avoid spam content, filter users with at most 20 tweets per day.\\
% 	\end{tabular}
% 	\label{tab:dataset-filter_policies}
% \end{table*}


\begin{figure}[t]
\centering
\includegraphics[width=0.92\columnwidth]{images/flow_v3.pdf}
% \includesvg[width=0.8\columnwidth]{imgs/flow-diagram.svg}
\caption{\small % Filtered data % inreply to tweet = false, retweet = false, tranced = flase, quoted tweet = false, daily tweets $\leq$ 20, follower $\geq$ 100k, verified = true, lang = en) 
% (e.g. no retweets/quoted tweets from users with $\geq$ 100k followers) 
%as basis for classifier and generator data set. Used models include pre-trained GPT and OPT versions.
Data pipeline used for modeling.
%Data pipeline (for filter policies cf. Tab.~\ref{tab:dataset-filter_policies}) used for models (e.g. pre-trained GPT versions). 
}
\label{fig:flowchart}
\end{figure}


==> main.tex <==



